3M: Multi-modal Multi-task Multi-teacher Learning for Game Event Detection

Esports has rapidly emerged as a global phenomenon with an ever-expanding audience via platforms, like YouTube. Due to the inherent complexity nature of the game, it is challenging for newcomers to comprehend what the event entails. The chaotic nature of online chat, the fast-paced speech of the game commentator, and the game-specific user interface further compound the difficulty for users in comprehending the gameplay. To overcome these challenges, it is crucial to integrate the Multi-Modal (MM) information from the platform and understand the event. The paper introduces a new MM multi-teacher-based game event detection framework, with the ultimate goal of constructing a comprehensive framework that enhances the comprehension of the ongoing game situation. While conventional MM models typically prioritise aligning MM data through concurrent training towards a unified objective, our framework leverages multiple teachers trained independently on different tasks to accomplish the Game Event Detection. The experiment clearly shows the effectiveness of the proposed MM multi-teacher framework.

==> chapters/relworks.tex <==


Previous works to enhance game comprehension include usage of additional visualisation tools via an additional smartphone medium \cite{kokkinakis2020dax}, or through additional overlays on the livestream screen to convey the notable performance of players \cite{block2018narrative}. 
Furthermore, there are also efforts focused on generating commentary by leveraging in-game data and video content using various deep learning models, ranging from seq2seq \cite{ishigaki-etal-2021-generating} to Transformers \cite{zhang-etal-2022-moba,tanaka-esports,wang2022esports}.
These approaches typically rely on data sources extracted solely from the game itself, utilising a single modality.

On the other hand, there exist investigations addressing the comprehension of livestream chat. 
Notable endeavours in this domain encompass the detection of toxic chat \cite{weld2021conda,kim2022understanding}, as well as examinations into the characteristics of conversational language \cite{ford2017chat}.
These explorations specifically delve into how the language in livestream chat deviates from conventional language grammar.
While prior research has contributed to an enhanced comprehension of both gaming dynamics and chat platforms, there remains a gap in the literature concerning the integration of livestream content and chat platforms together to establish a comprehensive understanding of the overall gaming situation.

Our method, therefore combines the multiple modalities, sourcing from both the game and audience reaction from the livestream platform to facilitate a model for game event detection. 



